Deep Learning for Effective and Efficient Reduction of Large Adaptation Spaces in Self-Adaptive Systems

Many software systems today face uncertain operating conditions, such as sudden changes in the availability of resources or unexpected user behavior. Without proper mitigation these uncertainties can jeopardize the system goals. Self-adaptation is a common approach to tackle such uncertainties. When the system goals may be compromised, the self-adaptive system has to select the best adaptation option to reconfigure by analyzing the possible adaptation options, i.e., the adaptation space. Yet, analyzing large adaptation spaces using rigorous methods can be resource- and time-consuming, or even be infeasible. One approach to tackle this problem is by using online machine learning to reduce adaptation spaces. However, existing approaches require domain expertise to perform feature engineering to define the learner, and support online adaptation space reduction only for specific goals. To tackle these limitations, we present 'Deep Learning for Adaptation Space Reduction Plus' -- DLASeR+ in short. DLASeR+ offers an extendable learning framework for online adaptation space reduction that does not require feature engineering, while supporting three common types of adaptation goals: threshold, optimization, and set-point goals. We evaluate DLASeR+ on two instances of an Internet-of-Things application with increasing sizes of adaptation spaces for different combinations of adaptation goals. We compare DLASeR+ with a baseline that applies exhaustive analysis and two state-of-the-art approaches for adaptation space reduction that rely on learning. Results show that DLASeR+ is effective with a negligible effect on the realization of the adaptation goals compared to an exhaustive analysis approach, and supports three common types of adaptation goals beyond the state-of-the-art approaches.

==> 3-research_goal.tex <==
\section{Research goal}\label{sec:research_goal}

A recently proposed approach to the adaptation space problem is reducing the adaptation space~\cite{quin2019efficient}. Adaptation space reduction aims at retrieving a subset of adaptation options from an adaptation space that contains only relevant system configurations that are then considered for analysis. An adaptation option is labeled relevant when it is predicted to satisfy the adaptation goals.

Existing work has showed that different machine learning techniques can be applied to reduce adaptation spaces, see for instance~\cite{elkhodary2010fusion, quin2019efficient, metzger2019feature, jamshidi2019machine}. Among the learning techniques that have been studied are decision trees, classification, regression, and online learning. However, current approaches only handle threshold goals, i.e., goals where a system parameter needs to stay below or above a given value. For instance, the throughput of a web-based system should not drop below a required level. For many practical systems today this is not sufficient as they also need to address optimization goals and set-point goals. For instance, minimize the operational cost of a web-based system, and maintain a constant energy consumption (to avoid peak loads on the electricity network) are respectively an optimization goal and a set-point goal

This leads to the following research goal:
\begin{quote}
\textit{Enable effective and efficient decision-making based on the various types of goals in self-adaptive systems.}
%\textit{How to reduce large adaptation spaces of self-adaptive systems with multiple threshold goals and/or a set-point goal and/or an optimization goal effectively?}
\end{quote}
With \textit{effective}, we mean the solution should ensure: \textbf{1)} the reduced adaptation space is significantly smaller, \textbf{2)} high performance, i.e., the reduced adaptation space covers the relevant adaptation options well, \textbf{3)} the effect of the state space reduction on the realization of the adaptation goals is negligible. With \textit{efficient} we mean the solution should ensure: \textbf{4)} the overhead time introduced by the learning approach is neglectable, \textbf{5)} there is no notable effect on 1, 2, 3 and 4 for larger sizes of the adaptation space.

Note that we explicitly use decision-making instead of adaptation space reduction. With decision-making we want to indicate that we focus not only on analysis, but reduce the adaptation space even further up to a decision, i.e., a ranking amongst the proposed adaptation options.

To answer the research goal, we propose a novel approach for adaptation space reduction
called ``Deep Learning for Adaptation Space Reduction Plus'' (DLASeR\fplus{}). This approach leverages deep learning to enable effective and efficient decision-making in self-adaptive systems. DLASeR\fplus{} is a general, extendable framework that performs effective adaptation space reduction for threshold, set-point and optimization goals. In this framework a deep learning neural network is maintained to cope with the dynamics of the system and its environment.

We explore deep learning for various reasons. 
First, considering that the (linear) machine learning models in previous work~\cite{quin2019efficient} add little additional training time, argues that deep learning might not introduce a large overhead either. 
Furthermore, classic learning techniques usually require feature engineering, whereas deep learning can handle raw data, i.e, meaningful features can be automatically learned and extracted, making feature engineering unnecessary.  
Next to this, learned features and even entire models can be reused across similar tasks. This is called transfer learning, and is a consequence of representation learning, which is basically the core concept that drives deep learning. We will exploit representation learning in our DLASeR\fplus{} neural network architecture. 
Finally, given the success of deep learning in various other domain, e.g., computer vision~\cite{russakovsky2015imagenet} and natural language processing~\cite{radford2019language}, we want to explore the applicability of deep learning for an important problem in self-adaptive-systems.

==> 5-metrics_backup.tex <==
\section{Metrics}\label{sec:metrics}
To answer the research question, we determined metrics that allow us to evaluate the different aspects of effectiveness and efficiency of the proposed solution. %DLASeR\fplus{}. 
Table~\ref{tab:metrics-research-question} summarizes the metrics.% for each aspect.

\begin{table}[htbp]
\toprule
\begin{tabular}{@{}ll@{}}
%\toprule
\multicolumn{2}{c}{\textbf{Effectiveness}} \\ \bottomrule
\multicolumn{1}{l|}{Coverage relevant adaptation options} & \begin{tabular}[c]{@{}l@{}}F1-score (for threshold and set-point goals)\\ Spearman's rho (for optimization goal)\end{tabular} \\ \hline
\multicolumn{1}{l|}{Reduction adaptation space} &  
\begin{tabular}[c]{@{}l@{}}Average adaptation space reduction (AASR) \\ Average analysis reduction (AANR)\end{tabular} \\ \hline
\multicolumn{1}{l|}{Effect on realization adaptation goals} & \begin{tabular}[c]{@{}l@{}}Differences in mean values of quality properties of \\ the goals with and without learning\end{tabular} \\ \toprule
\multicolumn{2}{c}{\textbf{Efficiency}} \\ \bottomrule
\multicolumn{1}{l|}{Learning time} & \begin{tabular}[c]{@{}l@{}}Time used for learning (fraction of s) \\ Time reduction for analysis with learning (\%)\end{tabular} \\ \hline
\multicolumn{1}{l|}{Scalability} & Metrics above for increasing size of adaptation space
\end{tabular}\bottomrule\vspace{10pt}
\caption{Left: different aspects of research question to be evaluated; right: metrics for each aspect.}
\label{tab:metrics-research-question}
\end{table}

We use different metrics to capture the coverage of relevant adaptation options for classification and regression. In particular, we use the F1-score for classification and Spearman's rank correlation coefficient (Spearman's rho) for regression.\footnote{A common metric to evaluate regression models is mean squared error (MSE). However, since we are more interested in the ranking of the regressed output, we use Spearman'rho to capture this ranking, which is not covered by MSE.} We define average adaptation space reduction (AASR) and average analysis reduction (AANR) to capture and compare the reduction of adaptation spaces. To capture the effect on the realization of the adaptation goals, we use the differences in mean values over time for the corresponding quality properties with and without learning. We measure the time used for learning and compare this with the time that would be necessary to analyze the complete adaptation space.  Finally, for scalability, we apply the different metrics for scenarios with an increasing size of adaptation spaces. We further elaborate on F1-score, Spearman's rho, AASR, and AANR. The other basic metrics are further explained in the evaluation section. 

\subsection{F1-score: precision and recall}
The quality of a classification algorithm is often expressed in terms of precision and recall. Applied to the classification of adaptation options (relevant or not relevant according to the adaptation goals), precision is the fraction of selected adaptation options that are relevant, while recall is the fraction of the relevant options that are selected from the total number of relevant options. Hence, precision and recall are a measure of relevance.
%
The F1-score combines both metrics with equal importance into a single number. Concretely, the F1-score is defined as the harmonic mean of precision and recall~\cite{geron2019hands}; 
\begin{equation}
    F1 = 2*\frac{precision * recall}{precision + recall}
\end{equation}

\subsection{Spearman correlation}
Spearman correlation, or Spearman's rho, is a non-parametric metric that can be used to measure rank correlation. We use this as a metric to capture the ranking of the predicted values of quality properties of regression models. The Spearman correlation essentially converts the predicted values to numeric ranks and then assesses how well a monotonic function describes the relationship between the predicted ranks and the true ranks. Spearman's rho is defined as~\cite{kokoska2000crc}:
\begin{equation} 
    \rho_{xy} = \frac{n \sum x_i y_i - \sum x_i \sum y_i}{\sqrt{n \sum x_i^2 - (\sum x_i)^2} \sqrt{n \sum y_i^2 - (\sum y_i)^2}}
\end{equation}
This formula computes the Spearman correlation between $x$ (the predictions of the selected adaptation options) and $y$ (the true values for the selected adaptation options), with $n$ the number of observations (the number of selected adaptation options). The result is a value between 0 and 1 (for an increasing monotonic trend, or -1 for a decreasing monotonic trend). Large errors are penalized harder. For example, a swapping of the first and third rank in the  prediction results is worse (lower Spearman's rho) compared to a swapping of the first and second rank. 


%Spearman correlation, also called Spearman's rho, is a useful non-parametric measure of rank correlation. We will use this metric to capture the ranking quality of regression ML models.  Spearman's rho simply converts the values of the predicted (regressed) quality to numeric ranks. Then, the linear relationship is calculated with the true ranks. This assesses how well a monotonic function describes the relationship between the predicted and the true ranks.  Spearman's rho is expressed as follows~\cite{kokoska2000crc}:
%\begin{equation} 
 %   \rho_{xy} = \frac{n \sum x_i y_i - \sum x_i \sum y_i}{\sqrt{n \sum x_i^2 - (\sum x_i)^2} \sqrt{n \sum y_i^2 - (\sum y_i)^2}}
%\end{equation}
%The above formula calculates the Spearman correlation between $x$ and $y$, with $n$ the number of observations. Large errors are penalized harder. For example, swapping the first and third rank in your prediction results in a worse association than if the first and second rank were swapped

\subsection{Average Adaptation Space Reduction}
To capture how well the adaptation space is reduced, we define a new metric called average adaptation space reduction ($AASR$).
%$AASR$ captures the percentage of adaptation options that are not considered relevant. 
$ASR$ (adaptation space reduction) is defined as: 
\begin{equation} 
    ASR = 1 - \frac{selected}{total}  
\end{equation}
with $selected$ the number of adaptation options selected by learning and $total$ the total number of adaptation options. 
%of the adaptation space. 
For instance, an adaptation space reduction of 70\% means that, after learning, only 30\% of the original adaptation space is considered for analysis. We obtain the average adaptation space reduction ($AASR$) by taking the average of the adaptation space reduction ($ASR$) over multiple adaptation cycles.
$AASR$ is a particularly suitable metric for stakeholders as it covers the high-end goal of adaptation space reduction.

%It is important to note that the interpretation of the relative adaptation space reduction depends on the types of adaptation goals considered. For threshold and set-point goals, the relative adaptation space reduction corresponds to the percentage of adaptation options that are predicted to conform with the given threshold and/or set-point goals. However, for an optimization goal, the relative adaptation space reduction corresponds to 100\% minus the percentage of adaptation options that have to be analyzed until an adaptation option is found that meets all the threshold and set-point goals. We explain this in detail in the next section. 

Remark that the average adaptation space reduction is determined by the system's adaptation goals. In particular, for the three types of goals considered in this work, the $AASR$ is determined by the threshold and set-point goals, corresponding to the percentage of adaptation options that are predicted to be conform with these goals. For systems with only optimization goals, the $AASR$ is zero (since the selected and total number of adaptation options are the same). 

%to 100\% minus the percentage of adaptation options that have to be analyzed until an adaptation option is found that meets all the threshold and set-point goals. We explain this in detail in the next section. 
%
It is also interesting to note that the $AASR$ depends on the restrictiveness of both threshold and set-point goals. Suppose that the threshold and set-point goals are not very restrictive, thus many adaptation options will comply with the adaptation goals. In this case, the reduction will be rather small. In the other case, for very restrictive threshold and set-point goals the opposite is true. A larger reduction for these goals can be expected. 
%, and a smaller reduction for only an optimization goal.


\subsection{Average Analysis Reduction}
To capture the effect of the adaptation space reduction on the effort required for analysis, we define a new metric called average analysis reduction ($AANR$). 
$ANR$ (analysis reduction) is defined as: 
\begin{equation} 
    ANR = 1 - \frac{analyzed}{selected}  
\end{equation}
with $analyzed$ the number of adaptation options that have been analyzed and $selected$ the number of adaptation options selected by learning. For instance, an analysis reduction of 90\% means that only 10\% of the adaptation options selected by learning were analyzed to find an option to adapt the system. We obtain the average analysis reduction ($AANR$) by taking the average of the analysis reduction ($ANR$) over multiple adaptation cycles.
Similarly to $AASR$, $AANR$ also covers a high-end goal of adaptation space reduction.

Note that the $AANR$ depends on the analysis approach that is used to find an adaptation option from the reduced adaptation space (and not on the constraints imposed by the adaptation goals as for $AASR$).   
In particular, the \textit{analysis reduction} corresponds to 100\% minus the percentage of selected adaptation options that have to be analyzed until an adaptation option is found that meets all the threshold and set-point goals.
For systems that include threshold, set-point and an optimization goal, the selected adaptation options are analyzed in the order predicted for the optimization goal. For systems with only threshold and set-point goals, the most basic method to analyze the selected adaptation options is by randomly picking (without replacement) one. For this specific case, we randomly shuffle the selected options in each cycle, resulting in a more representative $AANR$ score.
Remark that for systems with a large adaptation space and only an optimization goal, $AANR \approx 100$\% (since $analyzed$ is 1 and $selected$ is a large number equal to the size of the adaptation space).

